Reliability is Blind: Collective Incentives for Decentralized Computing Marketplaces without Individual Behavior Information

In decentralized cloud computing marketplaces, ensuring fair and efficient interactions among asset providers and end-users is crucial. A key concern is meeting agreed-upon service-level objectives like the service's reliability. In this decentralized context, traditional mechanisms often fail to address the complexity of task failures, due to limited available and trustworthy insights into these independent actors' individual behavior. This paper proposes a collective incentive mechanism that blindly punishes all involved parties when a task fails. Based on ruin theory, we show that Collective Incentives improve behavior in the marketplace by creating a disincentive for faults and misbehavior even when the parties at fault are unknown, in turn leading to a more robust marketplace. Simulations for small and large pools of marketplace assets show that Collective Incentives enable to meet or exceed a reliability target, i.e., the success-rate of tasks run using marketplace assets, by eventually discarding failure-prone assets while preserving reliable ones.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart

DEV=-dev # To switch dev on
#DEV=

PDF = $(PACKAGE).pdf acmguide.pdf

BIBLATEXFILES= $(wildcard *.bbx) $(wildcard *.cbx) $(wildcard *.dbx) $(wildcard *.lbx)
SAMPLEBIBLATEXFILES=$(patsubst %,samples/%,$(BIBLATEXFILES))

ACMCPSAMPLES= \
	samples/sample-acmcp-Discussion.pdf \
	samples/sample-acmcp-Invited.pdf \
	samples/sample-acmcp-Position.pdf \
	samples/sample-acmcp-Research.pdf \
	samples/sample-acmcp-Review.pdf \

all:  ${PDF} ALLSAMPLES

%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES: $(SAMPLEBIBLATEXFILES)
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/abbrev.bib: ACM-Reference-Format.bst
	perl -pe 's/MACRO ({[^}]*}) *\n/MACRO \1/' ACM-Reference-Format.bst \
	| grep MACRO | sed 's/MACRO {/@STRING{/' \
	| sed 's/}  *{/ = /' > samples/abbrev.bib 


samples/%.bbx: %.bbx
samples/%.cbx: %.cbx
samples/%.dbx: %.dbx
samples/%.lbx: %.lbx



samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex${DEV} $(notdir $<); done

samples/sample-sigconf-biblatex.pdf: samples/sample-sigconf-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex${DEV} $(notdir $<); done

samples/sample-acmsmall-biblatex.pdf: samples/sample-acmsmall-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex${DEV} $(notdir $<); done

samples/sample-sigconf-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex${DEV} $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex${DEV} $(notdir $<)
	cd $(dir $@) && xelatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex${DEV} $(notdir $<); done

samples/sample-sigconf-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex${DEV} $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex${DEV} $(notdir $<)
	cd $(dir $@) && lualatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex${DEV} $(notdir $<); done

samples/sample-acmcp.pdf: samples/acm-jdslogo.png

.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut \
	samples/acm-jdslogo.png \
	samples/*.run.xml samples/*.bcf $(SAMPLEBIBLATEXFILES)


clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

# distros
distros: all docclean
	zip -r acm-distro.zip  \
	acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.* \
	--exclude samples/sample-acmengage*
	zip -r acmengage-distro.zip samples/sample-acmengage* \
	samples/*.bib \
	acmart.pdf acmguide.pdf  *.cls ACM-Reference-Format.*

acmcp.zip: ${ACMCPSAMPLES} acmart.cls
	zip $@ $+

samples/sample-acmcp.tex: samples/samples.ins samples/samples.dtx
	cd samples; pdflatex samples.ins; cd ..


samples/sample-acmcp-%.tex: samples/sample-acmcp.tex samples/acm-jdslogo.png
	sed 's/acmArticleType{Review}/acmArticleType{$*}/' $< > $@

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

Version 2.06.  Added eISSN for a number of journals.
               ACM no longer collects or prints authors'
	       postal addresses

Version 2.05   Changed title for TELO.

Version 2.04   Compatibility with the new latex-dev format
               eSSN is always printed, even if pSSN is present
	       Wording change in copyright statement

Version 2.03   Cleaned generation of samples.
	       New options for printing conference proceedings
	       in ACM journals

Version 2.02   Documentation update.
	       Changes in TOG templates
	       Corrected typo in ACM/IMS journals

Version 2.01   \acmPrice now produces a warning.

Version 2.00   ACM switches to electronic only version.
	       We do not print article tabs anymore.
	       New copyright wording.
	       Deleted \acmPrice.

Version 1.93   Added PACMSE

Version 1.92   Documentation update
	       Emergency change: changed order of hyperref and hyperxmp
	       due to changes in the undelying packages

Version 1.91   Minor changes in ACMCP format

Version 1.90a  Changes in the sample keywords and concepts

Version 1.90   Journal ISSN updated

Version 1.89a  Added version info to .bst

Version 1.89   Bug fixes
	       Redesign of ACMCP
	       New positioning of badges
	       New journals: PACMMOD, TOPML

Version 1.88   New ISSNs
	       Documentation updates
	       New journal:  PACMNET

Version 1.87   CC license is allowed for non-acm documents and ACM Engage
	       documents only
	       New format acmcp for the cover page
	       New journals: JATS, ACMJCSS, TORS
	       Bug fixes

Version 1.86.  Empty country in affiliation now produces an error
               Bug fixes
	       New samples for acmengage

Version 1.85.  Bug fixes
	       Added support for Creative Commons licenses (requires
	       doclicense images)
	       New journals
	       New format acmengage for ACM Engage CSEdu course materials 

Version 1.84   Support for BibLaTeX rewritten (thanks to
	       Roberto Di Cosmo and Kartik Singhal)
	       Corrected German translation (thanks to Dirk Beyer)
	       New journals

Version 1.83   Support for multilanguage papers
	       ISSN changes for some journals

Version 1.82   Bug fixes.
	       New command \anon for anonymization of short strings.
	       Documentation update.

Version 1.81   Bug fixes
	       New bib field distinctURL to print URL even if doi is present.
	       Reworded samples

Version 1.80   New journals: DLT, FAC

Version 1.79   Fixed pages with index
	       (https://github.com/borisveytsman/acmart/issues/440)
	       Updated information for TAP, TCPS, TEAC

Version 1.78   Documentation update.
	       Magic texcount comments for samples.
	       Title page now is split if there are too many authors
	       Bug fixes.

Version 1.77   Changed the way to typeset multiple affiliations (Christoph Sommer)

Version 1.76   Added many journal abbreviations to the bst.
	       New experimental option: pbalance
	       ORCID linking code

Version 1.75   Omitted \country now produces error.
	       Added \AtBeginMaketitle

Version 1.74   Bug fixes.  A regression introduced in the font changes
	       is reverted.

Version 1.73   Bug fixes
	       The elements institution, city and country are now obligatory
	       for affiliations.  The absence of them produces a warning

Version 1.72   Bug fixes.  Better handling of metadata.

Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeLaTeX

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.63a   Moved TQUANT to TQC

Version 1.63	New journals: TQUANT, FACMP

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.52    Another rewording of licenses

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.49    New jorunal:  DTRAP

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.47    New journal: THRI

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.43    Bug fixes

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.41    Rearranged bib files
                Added new badges

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.39    Added \authornotemark commmand

Version 1.38    Increase default font size for SIGPLAN

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

Version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

Version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

Version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

Version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

Version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

Version 1.28    Bug fixes: natbib=false now behaves correctly.

Version 1.27    Bug fixes

Version 1.26    Bug fixes

Version 1.25    Updated PACMPL journal option.

Version 1.24    Added IMWUT journal option.

Version 1.23    Added PACM PL journal option.

Version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

Version 1.21    Bibliography changes: added arXiv, some cleanup

Version 1.20    Bug fixes, documentation updates

Version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

Version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.


Version 1.17    Formatting changes for margins and lists.  Bug fixes.

Version 1.16    Formatting changes for headers and footers.

Version 1.15    New structured affiliation command.
                New commands for acknowledgements.

Version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

Version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

Version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

Version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

Version 1.10    Bug fixes

Version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

Version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes


==> meta/indirections.tmpl.tex <==
\newcommand{\sysname}{Blind Slashing}
\newcommand{\figpatha}{example-image-a}
\newcommand{\figpathb}{example-image-b}
\newcommand{\figpathc}{example-image-c}
\newcommand{\figpathmodel}{example-image-a}
\newcommand{\figpatharch}{example-image-b}
\newcommand{\figpathattack}{example-image-c}
\newcommand{\figpathmotivation}{example-image-c}
\newcommand{\figpathadr}{example-image-a}
\newcommand{\figpathsentrq}{example-image-b}
\newcommand{\figpathnbsawt}{example-image-c}


==> problem_statement.tex <==
\section{Model \& problem statement}\label{sec:problem_statement}
\henry[\faCalendar*]{Speak in this section of game theoretic analysis of the platform showing no incentive to behave correctly ...}
We detail the model of decentralized cloud computing marketplace that we consider and formalize our system.

\subsection{Roles and interactions}

\matthieu[\faLightbulb]{Segment the model in an operational/market layer (assets + matchings) and a governance layer (who owns assets, who made asset matchings): that way, you may separate the intrinsic/cooperative asset behaviour (eg.
buggy/incompatible) from its owner's behaviour (eg.
attacks).
You can then define governance separately, eg., first a simple case, centralized honest total owner (eg.
Cloud Service Provider, iExec scheduler) that simply wants to maximize success, and as an extension the decentralized case, where asset owners may compete, anyone including asset owners can make matches, etc,...
In short, bipartite asset ownership graph (with archetypal cases of centralized total ownership, decentralized asset owners but distinct from matcher, and fully decentralized)}
% \matthieu[\done]{Regarding economic dimension, if relevant, textually separate actors' protocol behaviour (provide asset, match assets) from their objectives/incentives (make tasks succeed, make money, don't lose money).
% While requesters paying asset owners for successful tasks can be considered intuitive/expected behaviour, how to behave in case of failures is a design choice (eg.
% pay but reduce reputation, reimburse requester, slash everyone, etc, ...).}

In the decentralized computing system under study, various actors collaborate to perform tasks and produce outputs.
A task generally involves executing an application that uses various resources as inputs (those can be assets such as datasets or parameters) and delivers a result as its output.
% \matthieu[\done ?]{What's a task in a DCS? What's an output? Put down-to-earth intuitive descriptions at the start of the model description.
% If you lose people at this point, you won't recover them after.
% Same for what follows.} 
The process starts when a requester defines the required inputs.
The assets may include datasets, decentralized applications (dApps), or computing power, while the parameters could encompass computing specifications, and other requirements.
Once the request is made, the system identifies and allocates the appropriate assets and initiate execution.
Asset providers are usually compensated for supplying the requested resources.
As such, the primary goal for all parties should be to successfully complete tasks, ensuring a high success rate overall and securing their earnings.

% \matthieu[\done]{Regarding task sizes: iExec's task sizes are design choices.
% For genericity, in the model, one can also consider the requester as the "asset provider" of the task configuration/contract, which contains the task size (deadline), among others.
% In practice, it's closer to iExec, where a separate entity matches requesters' orders with providers' orders (technically anyone can trigger it).}
Operationally, this system can be modeled as a production function that incorporates multiple inputs, such as the requester, dataset, dApp, and computing provider, to generate an output.
Monitoring individual assets within this system is not possible as they ought to remain private, therefore the system does not provide detailed visibility into the performance or reliability of each input.
% \matthieu[\done]{Why is it costly? Is it even \textbf{feasible} in a decentralized trustless system?}
We operate in a "black box" scenario, where we are only aware of the selected inputs and the resulting output.
Over a series of tasks, the system’s role is to make sure that as many tasks as possible result in a successful output by filtering out problematic input or set of input.


In this system, an unsuccessful output can occur due to two primary reasons: one or more of the selected inputs may be faulty, either consistently or intermittently or the inputs themselves may be reliable, but certain combinations of them might be incompatible.
% \matthieu[\done]{are "unsuccessful output" and "resulting in a failure" significantly different? If not, only put one, to reduce the number of proposition is the already long sentence.}

\henry[\faQuestion]{Do we take into consideration the fact that there are different kind of assets, or do we generalize it to all of them being assets matched together ?}
\matthieu[\label{MB-c1}]{if we have an "(in)compatibility blackbox" that states which groups of assets can(not) work together (eg.
matching two assets, that happen to both be workerpools, won't work), n-ary any-to-any match-making encompasses the specific case where assets have types.
Can use asset typing as a real-world example, (or if genericity makes the formalization too complex...).
However, typing may be useful to distinguish hard incompatibilities (malformed request: two workers without workload), from soft incompatibilities (wellformed request, but wrong dataset format for the chosen dapp).
Prioritize readability..}
\henry[]{We will abstract the different kind of assets (datasets, dApps, computing) and consider that this is included in the incompatibility between two assets constraints.
The same way that a specific dApp may be incompatible with a specific worker, two assets being of the same type (a worker and another worker) are simply considered incompatible (cannot run a worker on a worker)}

\subsection{System formalization \& constraints}
We formalize the decentralized computing system as a production function $F$, which takes a set of $N_{a}$ inputs (where $N_{a} \geq 2$) and produces a corresponding output.
The system is defined by the function:

\begin{equation}
    y = F(a_1, a_2, \dots, a_{N_a})
    \label{eq:production-function}
\end{equation}

where $y$ represents the output, and $a_{1}, a_{2}, \dots, a_{N_{a}}$ are the various inputs required to generate this output.
These inputs correspond to different assets provided by actors within the system, such as the request, dataset, dApp, and computing power.
Each input can be linked back to its owner, and multiple inputs may share the same owner.

The production function $F$ will produce a successful output $y$ if two conditions are satisfied: first, none of the inputs $a_{i}$ are faulty at the time of execution; and second, no subset of inputs $(a_{i}, a_{j}, \dots)$ from the full set $(a_{1}, a_{2}, \dots, a_{N_a})$ is incompatible.
A subset of inputs is considered incompatible if, when used in the production function, it results in an unsuccessful output, even though all of its individual inputs are reliable.
% \matthieu[\done]{What if a dApp runs fine with small datasets on a weak-powered worker, but misses the deadline with larger datasets? It is not a necessarily dataset-worker incompatibility, because a better-complexity dApp may make the task succeed.
% Similarly, a more powerful worker, or smaller dataset, also work.
% So it's a "trio"-incompatibility.}

We model each set of one or more inputs as having an individual probability $p_{i}$ of being faulty.
Given these individual probabilities, we can compute the overall probability $P(y = \mathit{failure})$ of the output $y$ being unsuccessful.
However, the system operates as a "black box," so it does not provide detailed information on the internal reliability of each subset of inputs $(a_i, a_j, \dots)$.
Instead, the system only reveals the state of the final output $y$ and the selected full set of inputs $(a_{1}, a_{2}, \dots, a_{N_{a}})$.%\matthieu[\done]{What are the assumptions/the model for incompatible assets?}

\subsection{Building blocks}
We will now introduce the key components that serve as the groundwork for this work.

% \subsubsection{Staking and Slashing}
% In decentralized networks, staking and slashing mechanisms are fundamental tools used to incentivize honest behavior and ensure the reliability of participants.


% Staking involves participants locking up a certain amount of their assets, or tokens, as collateral to perform actions within the network, such as validating transactions, participating in consensus, or providing computational services.
% This stake serves as a security deposit, signaling the participant’s commitment to the network and their alignment with its goals.
% The higher the stake, the greater the incentive for the participant to behave honestly, as any malicious or faulty behavior could result in the loss of their staked assets.
% In return for staking, participants are often rewarded with network tokens or other benefits, encouraging long-term commitment and participation.

% Slashing is the counterpart to staking and serves as a penalty for dishonest or faulty behavior.
% If a participant is found to act maliciously or is involved in an activity that harms the network, a portion (or, in severe cases, all) of their staked assets is forfeited or "slashed." This punitive measure not only discourages harmful actions but also deters low-quality performance, such as submitting faulty computations or failing to properly validate transactions.
% Slashing is designed to balance rewards and penalties within the network.
% The severity of the slashing penalty typically depends on the severity of the offense, with harsher penalties for actions that pose greater risks to the network’s security or integrity.
% By creating a financial disincentive for dishonest behavior, slashing strengthens the network's resilience and ensures that participants are incentivized to follow protocol rules.

% In our work, we implemented staking and slashing as the incentive mechanism for the decentralized computing system, aiming to ensure cooperation and encourage positive behavior and contributions within the network.
% The key distinction in our approach, however, is that we face the challenge of not knowing who to slash directly.

% \subsubsection{Game theory \cite{binmore_game_2007}: Players, Strategies and Nash equilibrium}
% \matthieu[\plannedforlater]{*Theories* may be too broad to be building *blocks*, but individual algorithms/protocols proven correct under said theories may be building blocks}
% \matthieu[\plannedforlater]{For a real article, I do not think 20\% of a page about Game Theory will be relevant, same for ruin theory.
% A shorter explanation, of what we use from GT or RT and why (e.g., relevant assumptions/modelling power for our problem + what properties it gives us), seems more appropriate.
% Can be kept for the technical internship report, however.}

% Game theory is a mathematical framework for analyzing strategic interactions among rational decision-makers, referred to as players.
% Each player in a game selects a strategy, which is a predefined plan of action in response to various scenarios that may arise within the game.
% The outcome of the game is determined by the combination of strategies chosen by all players, and each player receives a payoff based on the resulting outcome.

% A fundamental concept within game theory is the Nash equilibrium, which occurs when all players have chosen their strategies, and no player can benefit by unilaterally changing their own strategy.
% At Nash equilibrium, each player's strategy is optimal, given the strategies of all other players.
% This concept is widely used to model and predict the behavior of participants in various competitive environments, from economics to biology.

% In our work, game theory is utilized to analyze the strategic behaviors of different actors within a decentralized cloud computing system, ensuring that the incentives are aligned to promote cooperation and reliability across the network.

% \subsubsection{Ruin theory \cite{asmussen_ruin_2010}: Ruin probability and Time of ruin}
% Ruin theory, originally developed within actuarial science, provides a mathematical framework for assessing the risk of a participant's financial collapse, or "ruin," over time.
% The primary focus of ruin theory is to investigate the probability that an insurer's surplus will eventually fall below zero, taking into account variables such as incoming cash premiums, premium rates, outgoing claims, and claims rates.
% Two key metrics in ruin theory are the ruin probability, which quantifies the likelihood of an entity’s capital depleting to zero or below, and the time of ruin, which estimates the expected time until this depletion occurs.

% In our paper, we compute ruin theory and time of ruin within the context of a blind slashing system for decentralized cloud computing to evaluate the probability of ruin for various asset owners, based on the reliability of their assets $p_{i}$.
% This approach enables the design of mechanisms that decrease the probability of ruin for reliable participants while increasing it for less reliable ones, thus enhancing the overall reliability and stability of the system.

\subsection{Threat model}
In the context of a decentralized cloud computing marketplace, the threat model can be divided into two key perspectives: the technical side, which focuses on potential system failures, and the actor side, which considers the behaviors and motivations of the participants that could trigger these failures.

\subsubsection{Motivations behind failure}
% On an actor standpoint, system failures can stem from both intentional and unintentional behaviors of the participating actors.
% These actors enjoy a high degree of flexibility: they can create multiple identities, join and leave the network freely, remain anonymous, and provide various inputs to the system.
% However, they are constrained by a limited budget, which means the scale of their actions—both benign and malicious is ultimately tied to their financial resources.
% The potential for system disruption is therefore proportional to the number and capability of actors involved.

% Actors may inadvertently introduce faulty inputs due to honest mistakes, lack of knowledge, or negligence.
% These unintentional errors can still pose a significant threat to system integrity, as they can lead to performance and reliability issues.
% Honest participants may, for example, submit inputs that are incorrectly configured, incompatible with other inputs, or simply misaligned with the system’s requirements.

% On the other hand, malicious actors pose an additional, more deliberate threat.
% Some may aim to disrupt the system, diminish trust in the marketplace, or gain a competitive advantage by orchestrating failures that benefit their own interests.
% Others may seek to exploit system vulnerabilities to damage the reputation of competing assets or to manipulate resource allocation and reliability assessments.
% They may inject inputs designed to cause failures, either consistently or under specific conditions.
% For instance, a decentralized application (dApp) could be intentionally engineered to fail only in certain scenarios, making it difficult to detect until the failure actually occurs.
% \matthieu[\done]{Is there something an attacker \textbf{can't} do? It is difficult to defend against fully arbitrary attackers.
% Note that using staking means that attackers do have some weaknesses, e.g., a limited attack budget.}

\subsubsection{Cause of failure}
% From a technical standpoint, the system is vulnerable to failures stemming from faulty inputs and incompatibility among inputs.
% One significant threat is the presence of faulty inputs, which can arise due to various reasons such as defects, malfunctions, or errors in the data, decentralized applications (dApps), or computing power provided by the system's assets.
% The assumption in our model is that a single faulty input is sufficient to trigger an unsuccessful output.
% Given that the system operates as a "black box," it is challenging to identify and rectify such faults without detailed internal monitoring.
% Faulty inputs can be consistently defective or intermittently problematic, making detection and resolution even more difficult.

% Another technical threat is the incompatibility of inputs.
% Even when all inputs are individually reliable, certain combinations may fail to interact correctly due to issues such as mismatched data formats, incompatible application logic, or resource conflicts.
% These incompatibilities can lead to failed executions, as the system lacks visibility into the internal interactions between different inputs.
% The model assumes that such incompatibilities inevitably result in failures, thereby posing a significant challenge to the overall reliability of the system.

% \subsection{Problem statement}
% In this section, we analyze the decentralized cloud computing system through the lens of game theory.
% We will examine how the strategic decisions of different actors impact the overall system reliability.
% We aim to show the necessity of incentives to shape participants' behavior and system outcomes.

% \subsubsection{Players and strategies}
% In the context of decentralized cloud computing, we will assume that the primary participants are Requesters, Asset Providers, and Computing Providers.
% Requesters are entities that need computational tasks to be performed, Asset Providers provide the tools and data required for computational tasks and Computing Providers execute the tasks as requested, using the assets provided.

% Each of these actors can adopt one of two strategies: S (successful completion of their task) or F (failure in the execution of their task).
% A task is considered successful only if all involved actors choose the S strategy.
% If any one or more participants choose F, the task fails, resulting in no reward for successful completion and potentially leading to penalties, especially under a slashing mechanism.
% This simplistic model helps in understanding how different strategies can influence the overall success or failure of tasks within the system.

% \subsubsection{Nash Equilibria Identification}
% We identified several Nash equilibria under different conditions.
% In the simplest scenario, where no penalties were applied, five distinct Nash equilibria were found.
% Out of these five, only one led to a successful outcome where all players adopted an honest strategy (S, S, S), resulting in the successful completion of tasks.
% The remaining four equilibria were associated with failure, where at least one player adopted a non-cooperative (malicious or faulty) strategy, leading to negative outcomes for all involved.

% This analysis highlighted a key issue: while the (S, S, S) equilibrium is desirable, the presence of multiple equilibria with failure outcome means that players can easily slip and stay into non-successful strategies without strong incentives to move to a reliable and successful strategy.

% \subsubsection{Repeated Games and Cooperation}
% In repeated games, the potential for future interactions encourages cooperation among players.
% So we may expect strategies to shift toward a successful strategy over several games.
% However, the current system’s lack of penalties for non-cooperation allows players to remain in faulty strategies without significant repercussions.
% And even though the successful strategy is pareto superior, players have no incentive to switch as quickly as possible to a successful strategy.
% This is particularly problematic for Computing Providers, who are financially penalized even when others cause task failures.

% \subsubsection{Conclusion from Game Theory}
% Our game-theoretic analysis revealed significant issues in the incentive structures within the system.
% Although the (S, S, S) strategy is theoretically stable, undesired Nash equilibria persist, allowing players to adopt non-cooperative strategies without facing sufficient penalties.
% To address these problems, we propose a \sysname model, where all actors involved in a task face penalties upon its failure.
% This model would encourage cooperation, as all participants would have a direct financial stake in the success of each task and would therefore need to shift as quickly as possible to a successful strategy to not get ruined.

